PD-MORL: Preference-Driven Multi-Objective Reinforcement Learning Algorithm

Multi-objective reinforcement learning (MORL) approaches have emerged to tackle many real-world problems with multiple conflicting objectives by maximizing a joint objective function weighted by a preference vector. These approaches find fixed customized policies corresponding to preference vectors specified during training. However, the design constraints and objectives typically change dynamically in real-life scenarios. Furthermore, storing a policy for each potential preference is not scalable. Hence, obtaining a set of Pareto front solutions for the entire preference space in a given domain with a single training is critical. To this end, we propose a novel MORL algorithm that trains a single universal network to cover the entire preference space scalable to continuous robotic tasks. The proposed approach, Preference-Driven MORL (PD-MORL), utilizes the preferences as guidance to update the network parameters. It also employs a novel parallelization approach to increase sample efficiency. We show that PD-MORL achieves up to 25% larger hypervolume for challenging continuous control tasks and uses an order of magnitude fewer trainable parameters compared to prior approaches.

==> files/Rebuttal.tex <==
\newpage
\section{Response to Reviewer QTgN}
We thank the reviewer for their time and effort and address their concerns.

**C1:** The envelope Q-learning algorithm by Yang et al. is only compared in DST and FTN but missing from MuJoCo environments.

**A1:** As the reviewer stated, we showed that PD-MORL is superior to the Envelope approach in simpler environments with discrete action spaces, DST and FTN. The authors who proposed the Envelope algorithm have not evaluated it using the MuJoCo environments. All the environments used in their paper have discrete action spaces.
Therefore, the implementation for continuous action spaces is missing.
We also believe that the Envelope approach is not scalable to benchmarks with continuous action spaces such as MuJoCo environments.
Since PD-MORL outperforms the envelope algorithm even in simpler environments, its benefits on more complex problems with continuous action spaces are expected to be higher.

Our original justification in Section 5.2 may not have been clear. We clarified our choice as follows:

"We compare the performance of PD-MORL against two state-of-the-art approaches (Xu et al., 2020;
Chen et al., 2019) that use these continuous control benchmarks. 
We emphasize that these approaches must learn a different policy network for every solution on the Pareto front.
In contrast, PD-MORL learns a single universal network that covers the entire preference space.
The Envelope algorithm (Yang et al., 2019) is not included in these comparisons since it was not evaluated with continuous action spaces, and PD-MORL already outperforms it on simpler problems."


% We also believe that the Envelope approach is not scalable to benchmarks with continuous action spaces such as MuJoCo environments. In fact, in their work, all of the evaluated benchmarks have discrete action spaces.
% Although they provide an implementation of Envelope MOA3C, it is rather specific to the Multi-Objective SuperMario environment which is an image-based, discrete-action space environment. Therefore, the implementation for continuous action spaces are missing.

% Since many real-world tasks involve continuous state and action space, we showed the superior performance of PD-MORL to the Envelope approach using simple discrete benchmarks and further compare it with more recent MORL approaches using continuous control tasks. 


**C2:** Another important baseline is the conditional network with diverse experience replay algorithm in Abels et al. (Dynamic Weights in Multi-Objective Deep Reinforcement Learning). 

**A2:** We thank the reviewer for pointing out the work by Abels et al. 2019. We are aware of this work and have already mentioned it in the main manuscript in Sections 2 and 5. In their work, Yang et al. 2019, shows the superiority of the Envelope algorithm over the CN+DER approach provided by Abels et al.. Therefore, we only included the CN+DER approach as a comparison point in Appendix B.4 Table 7 regarding the CRF1 metric.

Additionally, Abels et al. evaluate their work only on image-based simple problems with discrete action spaces (Deep Sea Treasure and Minecart). This and the fact that their network architecture is based on Q-network suggest that their approach cannot be extended to problems with continuous action spaces such as MuJoCo environments.

**C3:** There seems to be a mismatch between the practical version of the algorithm and the theoretical version. Algorithm 1 uses the interpolated preference rather than the raw preference. Can the authors comment on this choice and how the theoretical result extends to this different update rule?

**A3:** We thank the reviewer for pointing out the potential confusion between the practice and theory regarding the use of projected preference in the optimality operator. 
The proof of Theorem 3 in Appendix A.2 assumes that an action $a^{\prime}$ is the action that maximizes $S_c(\boldsymbol{\omega},\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega}))\cdot(\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega}))$. This assumption is valid for projected preference $\boldsymbol{\omega}_p$. Therefore, the theoretical results extend this practical modification.
To avoid any confusion, we have also added the following sentence to "Preference alignment" paragraph in Section 4.2:

"This practical modification extends to theoretical results as the proof for Theorem 3 is also valid for $\boldsymbol{\omega}_p$."

% Additionally, the proof is given for multi-objective Q-learning which is based on Banach's Fixed-Point Theorem. However, in practice, Q-values are generally approximated using neural networks. This eventually may affect the consistence between practice and theory.

**C4:** There are some details missing in the description of the algorithm. The preference interpolation is an important part of the algorithm but its description is lacking. I suggest having a more detailed exposition on this, including how the key preference points are selected, how the normalization procedure is done, and a mathematical expression of the interpolation function.
  
**A4:** Based on the reviewers' suggestions, we have revised the "Preference alignment" paragraph in Section 4.2 to let the readers better understand the details of our algorithm in the main manuscript. These details were described before only in the Appendix B.1.3.
We further provide an additional reference for the radial basis function interpolator used in our work for interested readers in Appendix B.1.3.
The modifications/additions to the original manuscripts are highlighted in blue in the revised manuscript. 

**C5:** I have one question about using the cosine similarity in the preference-driven optimality operator. The cosine similarity is closely related to the inner product of the preference vector and the Q value vector, which is also in the operator itself. So is it really important to have the $\omega^TQ(s',a',\omega)$ term in the update rule, or is the cosine similarity itself sufficient?
  
**A5:** We thank the reviewer for pointing out this confusion of redundancy. 

Without the cosine similarity term, the supremum operator yields the action that only maximizes $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$. This may pull the target Q-values in the wrong direction, especially when the scales of the objectives are in different orders of magnitude. For instance, let us assume a multi-objective problem with percent energy efficiency ($\in [0, 1]$) being the first objective and the latency ($\in [1, 10]$) in milliseconds being the second objective. Let us also assume that the preference vector ($\boldsymbol{\omega} =$ \{$0.9, 0.1$\}) favors the energy efficiency objective and there are two separate actions ($a_1, a_2$) that yields Q-values of $Q_1 =$\{$0.9, ~1$\}, $Q_2 = $\{$0.1, ~10$\} respectively. The supremum operator chooses action, $a_2$ since $\boldsymbol{\omega}^T Q_2=1.09$ is higher than $\boldsymbol{\omega}^T Q_1=0.91$. Since the scales of these two objectives are in different orders of magnitudes, $\sup_{\substack{a^{\prime}\in A}}(\boldsymbol{\omega}^T\mathbf{Q}s^\prime,a^{\prime},\boldsymbol{\omega}))$ always chooses the action that favors the latency objective. This behavior negatively affects the training since the target Q-values are pulled in the wrong direction.
On the contrary, our novel cosine similarity term enables the optimality operator to choose actions that align the preferences with the Q-values and maximize the target value at the same time. The supremum operator now chooses action, $a_1$ since $S_c\cdot\boldsymbol{\omega}^T Q_1=0.75\times0.91 = 0.68$ is higher than $S_c\cdot\boldsymbol{\omega}^T Q_2=0.12\times1.09=0.13$. With this addition, the algorithm disregards the large  $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$ where the preference vector and the Q-values are not aligned since the $S_c(\boldsymbol{\omega},\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega}))$ takes small values.

We have added this detailed explanation of the benefit of using cosine similarity term in Section 4.2 after Equation 6. 
The modifications/additions to the original manuscripts are highlighted with blue in the revised manuscript.

**C6:** In theorem 4, the authors should define what $\mathbf{Q}^*$ is as it is not clear in the multi-objective setting.

**A6:** We thank the reviewer for pointing out the absence of the definition of $\mathbf{Q}^*$. The definition of $\mathbf{Q}^*$ was given in Appendix A.2; however, it was missing in the main manuscript. We have revised the main manuscript and stated explicitly that $\mathbf{Q}^*$ is the unique fixed point, the optimum Q-value for a given preference.      

\section{Response to Reviewer Mx6C}
We thank the reviewer for their time, effort and supportive review.

**C1:** Effectiveness of cosine similarity term.
  
**A1:** We thank the reviewer for pointing out this confusion of redundancy. 

Without the cosine similarity term, the supremum operator yields the action that only maximizes $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$. This may pull the target Q-values in the wrong direction, especially when the scales of the objectives are in different orders of magnitude. For instance, let us assume a multi-objective problem with percent energy efficiency ($\in [0, 1]$) being the first objective and the latency ($\in [1, 10]$) in milliseconds being the second objective. Let us also assume that the preference vector ($\boldsymbol{\omega} =$ \{$0.9, 0.1$\}) favors the energy efficiency objective and there are two separate actions ($a_1, a_2$) that yields Q-values of $Q_1 =$\{$0.9, ~1$\}, $Q_2 = $\{$0.1, ~10$\} respectively. The supremum operator chooses action, $a_2$ since $\boldsymbol{\omega}^T Q_2=1.09$ is higher than $\boldsymbol{\omega}^T Q_1=0.91$. Since the scales of these two objectives are in different orders of magnitudes, $\sup_{\substack{a^{\prime}\in A}}(\boldsymbol{\omega}^T\mathbf{Q}s^\prime,a^{\prime},\boldsymbol{\omega}))$ always chooses the action that favors the latency objective. This behavior negatively affects the training since the target Q-values are pulled in the wrong direction.
On the contrary, our novel cosine similarity term enables the optimality operator to choose actions that align the preferences with the Q-values and maximize the target value at the same time. The supremum operator now chooses action, $a_1$ since $S_c\cdot\boldsymbol{\omega}^T Q_1=0.75\times0.91 = 0.68$ is higher than $S_c\cdot\boldsymbol{\omega}^T Q_2=0.12\times1.09=0.13$. With this addition, the algorithm disregards the large  $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$ where the preference vector and the Q-values are not aligned since the $S_c(\boldsymbol{\omega},\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega}))$ takes small values.

We have added this detailed explanation of the benefit of using cosine similarity term in Section 4.2 after Equation 6. 
The modifications/additions to the original manuscripts are highlighted with blue in the revised manuscript.

We also note that, we already had an ablation study where we remove the cosine similarity term from the loss function in Appendix B.4 for continuous control tasks. In this section, we have discussed the results on this ablation study. 




\section{Response to Reviewer scaX}

We thank the reviewer for their time, effort, and supportive review. We want to emphasize that all the points the reviewer pointed out are towards improving the quality of this work, and we appreciate it. The modifications/additions to the original manuscripts are highlighted in blue in the revised manuscript.

**C1:** First, MORL benchmarks used are not very well explained and the visualizations for the tasks and policies are not very clear. I have minimal understanding of what the challenges in each benchmark are and why baselines failed in these tasks -- this paper does not need an exhaustive description of these benchmarks but could certainly explain them and the learned policies better through some textual revisions and more figures (e.g., fig 3 is not very well explained/useful in its current state). 

**A1:** We provide additional details for benchmarks in Sections 5.1 and 5.2. We also refer to Appendix B.2. at the beginning of Section 5 to lead the readers to detailed descriptions of the benchmarks used in this work.
As the reviewer suggested, we modified the second paragraph of Section 5.1, where we explain and refer to Figure 3 as follows:

"Figure 3 illustrates the policies achieved by PD-MORL for three preference vectors capture corner
cases. Although our policy is not specific to any preference, the submarine achieves optimal treasure
values for the given preference. For example, it finds the best trade-off within the shortest time (one step) when we only value the time penalty ($w=\{0,1\}$). As the importance of the treasure value increases 
($w=$\{0.5,0.5\}, $w=\{1,0\}$), it spends optimal amount of time (8 steps and 19 steps, respectively) to find a deeper treasure. "

**C2:** Next, the experimental results are not sufficiently explored. For example, the paper does not address why the contributed PD-MORL performs significantly worse than PG-MORL in the hopper experiment, or why sparsity is sometimes worse than PG-MORL. Including these results is essential, but so is some analysis insight into the weaknesses of PD-MORL relative to PG-MORL in these test cases, and perhaps also some ideas on how these issues in PD-MORL might be overcome. It also seems worth including some discussion on the limitations of these metrics.

**A2:** We agree with the reviewer that a more detailed discussion of the experimental results is missing. We have revised the third paragraph in Section 5.2 to address the reviewer's concerns and added a discussion as follows:

"We also note that PG-MORL achieves better sparsity metric for MO-HalfCheetah-v2 and MO-Ant-v2 environments. However, PG-MORL also achieves smaller hypervolume compared to PD-MORL. 
This suggests that to determine the quality of a Pareto front, these metrics are rather limited and should be further investigated by the existing literature. Therefore, we also plot Pareto front plots for all algorithms in Figure 5(a)-(e) to have a better understanding of the quality of the Pareto front."

"PD-MORL mostly relies on the interpolation procedure before the actual training. The key solutions obtained during this period determine the initial convergence of the algorithm. However, for MO-Hopper-v2, the obtained key solutions for preference vectors $\{1,0\}, \{0.5,0.5\}, \{0,1\}$ are $\{1778,4971\}, \{1227, 1310\}, \{3533, 3165\}$ respectively.
These key solutions are not a good representative of the Pareto front shown in Figure 5(e).
To have representative key solutions is a limitation to PD-MORL; however, it can be solved with hyperparameter tuning."

**C3:** On a related note, the results in Table 1 should have error values representing.

**A3:** Since these benchmarks are relatively simpler than the continuous control tasks, we specifically reported the mean values over different seeds in Table 1 and Table 7. The results are extremely similar using different seeds. 

**C4:** Thirdly, the usage of the cosine similarity in eq. 5 is not well enough explained -- the inner product of omega and Q should already reflect the cosine similarity of omega and Q(s,a, omega), so why is the scalar Sc(omega, Q) also multiplied by the inner product of omega and Q? 

**A4:** We thank the reviewer for pointing out this confusion of redundancy. 

Without the cosine similarity term, the supremum operator yields the action that only maximizes $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$. This may pull the target Q-values in the wrong direction, especially when the scales of the objectives are in different orders of magnitude. For instance, let us assume a multi-objective problem with percent energy efficiency ($\in [0, 1]$) being the first objective and the latency ($\in [1, 10]$) in milliseconds being the second objective. Let us also assume that the preference vector ($\boldsymbol{\omega} =$ \{$0.9, 0.1$\}) favors the energy efficiency objective and there are two separate actions ($a_1, a_2$) that yields Q-values of $Q_1 =$\{$0.9, ~1$\}, $Q_2 = $\{$0.1, ~10$\} respectively. The supremum operator chooses action, $a_2$ since $\boldsymbol{\omega}^T Q_2=1.09$ is higher than $\boldsymbol{\omega}^T Q_1=0.91$. Since the scales of these two objectives are in different orders of magnitudes, $\sup_{\substack{a^{\prime}\in A}}(\boldsymbol{\omega}^T\mathbf{Q}s^\prime,a^{\prime},\boldsymbol{\omega}))$ always chooses the action that favors the latency objective. This behavior negatively affects the training since the target Q-values are pulled in the wrong direction.
On the contrary, our novel cosine similarity term enables the optimality operator to choose actions that align the preferences with the Q-values and maximize the target value at the same time. The supremum operator now chooses action, $a_1$ since $S_c\cdot\boldsymbol{\omega}^T Q_1=0.75\times0.91 = 0.68$ is higher than $S_c\cdot\boldsymbol{\omega}^T Q_2=0.12\times1.09=0.13$. With this addition, the algorithm disregards the large  $\boldsymbol{\omega}^T\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega})$ where the preference vector and the Q-values are not aligned since the $S_c(\boldsymbol{\omega},\mathbf{Q}(s^\prime,a^{\prime},\boldsymbol{\omega}))$ takes small values.

We added this detailed explanation of the benefit of using cosine similarity term in Section 4.2 after Equation 6. 
The modifications/additions to the original manuscripts are highlighted with blue in the revised manuscript.

**C5:** I also don't fully understand the preference alignment procedure, including how the normalized solutions in Fig 2b are formed and what purpose there is to interpolating them, e.g. rather than interpolating in a different space.

**A5:** Most of the missing details were provided in the Appendix. Based on the reviewers' suggestions, we have revised the "Preference alignment" paragraph in Section 4.2 to let the readers better understand the details of our algorithm in the main manuscript. 

**C6:** Finally, the related works and experiments sections are rather monolithic and would benefit greatly from splitting the large paragraphs into individual ideas or techniques, possibly using other methods (e.g. figures/tables and subsections) to better organize and discuss the ideas in them.

**A6:** Since we added new details in the revised manuscript, we condensed some of the sections to eliminate the monolithic nature of these sections.

**C7:** The vector nature of Q is not well explained (why is the dimensionality of Q(s, a, w) equal to L and what does it represent before/after taking the inner product with omega?).

**A7:** The vector of nature Q is first introduced in the Background section, and L is an arbitrary choice of dimension. Similarly, in the same section, we explained the scalar nature of the inner product. These details are also provided in Appendix A.

**C8:** The walker results in fig 5 need y-axis labels

**A8:** We have added x-axis and y-axis labels to Figure 5.

**C9:** The paper should justify why fewer parameters is a big deal, the limitations/future work discussion isn't very interesting/compelling and should be more specific and try to offer some deeper insights.

**A9:** In the MORL community, the multi-objective nature of the algorithm is generally motivated by the fact that real-world tasks have multiple, possibly conflicting objectives. However, in order for them to be practical, MORL approaches should be deployable in real-world scenarios. Hence, they should be memory-efficient and energy-efficient. Using this insight, we have revised the third paragraph in Section 5.2 and added the following sentence:

"This may enable the deployment of PD-MORL in real-life scenario where there are dynamic changes in the design constraints and goals.


**C10:** Also, the use of L2 distance in sparsity is possibly worth discussing if there's space -- it seems like a rather arbitrary choice of metric so I am curious if there is a reason for it.

**A10:** We thank the reviewer for discussing the use of L2 distance in sparsity. We agree with the reviewer that L2 distance has its own limitations, especially when the objective space have large dimensions. However, we employ this metric to have a fair comparison with the existing literature.

We have revised the third paragraph in Section 5.2 and state that "to determine the quality of a Pareto front, these metrics are rather limited and should be further investigated by the existing literature." in the revised manuscript.

\section{Response to Reviewer sFJy}

We thank the reviewer for their time, effort and supportive review. 

**C1:** Some details are lacking in Section 4.2, specifically concerning the division of the preference space, the preference alignment using normalization and more importantly the extension of the algorithm to continuous action space. While it is true that these details are provided in the supplementary material, it would be helpful to have some hints in the main text. Space could be saved by condensing the introduction and related work section, which are rather detailed, thus leaving more space to describe the main novel components of this work.

**A1:** As the reviewer suggested, we have revised Section 4.2 to let the readers better understand the details of our algorithm in the main manuscript. Specifically, we have added

* A detailed explanation of the benefit of the cosine similarity term in the optimality operator in Section 4.2 after Equation 6.

* A hint on why HER is preferred in the second paragraph of Section 4.2.

* A more detailed explanation of the preference alignment procedure in the "Preference alignment" paragraph of Section 4.2.

* A more detailed explanation of MO-TD3-HER extension for continuous action space in the "Extension to continuous action space" paragraph of Section 4.2.

The modifications/additions to the original manuscripts are highlighted with blue in the revised manuscript.

**C2:** Small comments and typos:

**A2:** We also fixed the typos in the revised manuscript.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

